A Diffusion model for POI recommendation

Next Point-of-Interest (POI) recommendation is a critical task in location-based services that aim to provide personalized suggestions for the user's next destination. Previous works on POI recommendation have laid focused on modeling the user's spatial preference. However, existing works that leverage spatial information are only based on the aggregation of users' previous visited positions, which discourages the model from recommending POIs in novel areas. This trait of position-based methods will harm the model's performance in many situations. Additionally, incorporating sequential information into the user's spatial preference remains a challenge. In this paper, we propose Diff-POI: a Diffusion-based model that samples the user's spatial preference for the next POI recommendation. Inspired by the wide application of diffusion algorithm in sampling from distributions, Diff-POI encodes the user's visiting sequence and spatial character with two tailor-designed graph encoding modules, followed by a diffusion-based sampling strategy to explore the user's spatial visiting trends. We leverage the diffusion process and its reversed form to sample from the posterior distribution and optimized the corresponding score function. We design a joint training and inference framework to optimize and evaluate the proposed Diff-POI. Extensive experiments on four real-world POI recommendation datasets demonstrate the superiority of our Diff-POI over state-of-the-art baseline methods. Further ablation and parameter studies on Diff-POI reveal the functionality and effectiveness of the proposed diffusion-based sampling strategy for addressing the limitations of existing methods.

==> tables/main_result.tex <==

\begin{table}
\centering
\caption{The test results of \method{} and all baselines, where R@K and N@K are short for Recall@K and NDCG@K. The highest performance is emphasized with bold font and the second highest is marked with underlines.\textbf{$\star$} indicates that \method{} outperforms the best baseline model at the significance level with a p-value<0.05 level of unpaired t-test.}
\label{tab:overall}
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|cc|c}
\toprule %\hline
\multicolumn{10}{c}{\textbf{Gowalla}} \\
\bottomrule \hline \hline
Metrics & MF & LightGCN & DGCF & GeoIE & LSTPM & STAN & SGRec & DRAN & \method{}\\% & Improv. \\

\hline
Recall@2 & 0.0414 & 0.1802 & 0.1147 & 0.1767 & 0.1904 & \underline{0.2195} & 0.1932 & 0.2133 & \textbf{0.2635\textsuperscript{$\star$}} \\%& 20.0\% \\
Recall@5 & 0.0869 & 0.1348 & 0.1396 & 0.2123 & 0.2049 & 0.2364 & 0.2286 & \underline{0.2466} & \textbf{0.3086\textsuperscript{$\star$}} \\
Recall@10 & 0.1473 & 0.1699 & 0.1721 & 0.2436 & 0.2618 & 0.2994 & 0.2718 & \underline{0.3056} & \textbf{0.3421\textsuperscript{$\star$}} \\
\hline
NDCG@2 & 0.0428 & 0.0914 & 0.0995 & 0.1670 & 0.1431 & 0.1917 & 0.1573 & \underline{0.2038} & \textbf{0.2527\textsuperscript{$\star$}} \\
NDCG@5 & 0.0810 & 0.1162 & 0.1319 & 0.1829 & 0.1588 & 0.2152 & 0.1662 & \underline{0.2168} & \textbf{0.2716\textsuperscript{$\star$}} \\
NDCG@10 & 0.1078 & 0.1432 & 0.1561 & 0.1929 & 0.1742 & 0.2268 & 0.1704 & \underline{0.2367} & \textbf{0.2872\textsuperscript{$\star$}} \\
\bottomrule % \hline
\end{tabular}
}

\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|cc|c}
\toprule %\hline
\multicolumn{10}{c}{\textbf{Singapore}} \\
\bottomrule \hline \hline
Metrics & MF & LightGCN & DGCF & GeoIE & LSTPM & STAN & SGRec & DRAN & \method{}\\% & Improv. \\

\hline
Recall@2 & 0.1103 & 0.1606 & 0.1798 & 0.2521 & 0.2704 & 0.2634 & 0.3058 & \underline{0.3086} & \textbf{0.3455\textsuperscript{$\star$}} \\
Recall@5 & 0.1766 & 0.2144 & 0.2040 & 0.2867 & 0.3253 & 0.2940 & 0.3507 & \underline{0.3554} & \textbf{0.3906\textsuperscript{$\star$}} \\
Recall@10 & 0.2059 & 0.2419 & 0.2285 & 0.3162 & 0.3791 & 0.3280 & 0.3884 & \underline{0.3921} & \textbf{0.4294\textsuperscript{$\star$}} \\
\hline
NDCG@2 & 0.0744 & 0.1720 & 0.1973 & 0.2428 & 0.2610 & 0.2831 & 0.2274 & \underline{0.2972} & \textbf{0.3316\textsuperscript{$\star$}}  \\
NDCG@5 & 0.0791 & 0.1789 & 0.2162 & 0.2583 & 0.2697 & 0.2995 & 0.2697 & \underline{0.3175} & \textbf{ 0.3518\textsuperscript{$\star$}}  \\
NDCG@10 & 0.0868 & 0.1892 & 0.2269 & 0.2679 & 0.2749 & 0.2892 & 0.2916 & \underline{0.3297} & \textbf{0.3643\textsuperscript{$\star$}} \\
\bottomrule % \hline
\end{tabular}
}


\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|cc|c}
\toprule %\hline
\multicolumn{10}{c}{\textbf{Tokyo}} \\
\bottomrule \hline \hline
Metrics & MF & LightGCN & DGCF & GeoIE & LSTPM & STAN & SGRec & DRAN & \method{}\\% & Improv. \\

\hline
Recall@2 & 0.2896 & 0.3917 & 0.4204 & 0.4975 & 0.5029 & 0.5105 & 0.5091 & \underline{0.5225} & \textbf{0.6031\textsuperscript{$\star$}} \\
Recall@5 & 0.3141 & 0.4473 & 0.4913 & 0.5408 & 0.5513 & 0.5489 & 0.5488 & \underline{0.5570} & \textbf{0.6401\textsuperscript{$\star$}} \\
Recall@10 & 0.3866 & 0.4936 & 0.5310 & 0.5726 & 0.5795 & 0.6167 & 0.6173 & \underline{0.6210} & \textbf{0.6681\textsuperscript{$\star$}}\\
\hline
NDCG@2 & 0.1984 & 0.4207 & 0.4299 & 0.4842 & 0.4724 & 0.4990 & 0.4715 & \underline{0.5089} & \textbf{0.5886\textsuperscript{$\star$}} \\
NDCG@5 & 0.2071 & 0.4354 & 0.4376 & 0.5037 & 0.4881 & 0.5264 & 0.4905 & \underline{0.5390} & \textbf{0.6062\textsuperscript{$\star$}} \\
NDCG@10 & 0.2327 & 0.4403 & 0.4558 & 0.5141 & 0.4962 & 0.5554 & 0.5112 & \underline{0.5602} & \textbf{0.6160\textsuperscript{$\star$}} \\
\bottomrule % \hline
\end{tabular}
}

\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|cc|c}
\toprule %\hline
\multicolumn{10}{c}{\textbf{New York City}} \\
\bottomrule \hline \hline
Metrics & MF & LightGCN & DGCF & GeoIE & LSTPM & STAN & SGRec & DRAN & \method{} \\%& Improv. \\

\hline
Recall@2 & 0.2361 & 0.3789 & 0.3368 & 0.5655 & 0.5754 & \underline{0.6027} &  0.5734 & 0.5859 & \textbf{0.6589\textsuperscript{$\star$}} \\
Recall@5 & 0.2792 & 0.4363 & 0.4167 & 0.5994 & 0.6020 & \underline{0.6358} & 0.6175 & 0.6253 & \textbf{0.6755\textsuperscript{$\star$}} \\
Recall@10 & 0.3046 & 0.4519 & 0.5653 & 0.6251 & 0.6312 & \underline{0.6533} & 0.6424 & 0.6478 & \textbf{0.6884\textsuperscript{$\star$}} \\
\hline
NDCG@2 & 0.2002 & 0.3819 & 0.4847 & 0.5629 & 0.5524 & \underline{0.5887} & 0.5490 & 0.5702 & \textbf{ 0.6536\textsuperscript{$\star$}}   \\
NDCG@5 & 0.2318 & 0.3867 & 0.4922 & 0.5716 & 0.5596 & \underline{0.6092} & 0.5559 & 0.5881 & \textbf{0.6616\textsuperscript{$\star$}}   \\
NDCG@10 & 0.2426 & 0.3903 & 0.5041 & 0.5805 & 0.5681 & \underline{0.6124} & 0.5613 & 0.5956 & \textbf{0.6745} \\
\bottomrule % \hline
\end{tabular}
}

\end{table}


% \begin{table*}
% \centering
% \caption{The test results of \method{} and all baselines, where R@K and N@K are short for Recall@K and NDCG@K. The highest performance is emphasized with bold font and the second highest is marked with underlines.\textbf{$\star$} indicates that \method{} outperforms the best baseline model at a p-value<0.05 level of unpaired t-test.}
% \label{tab:overall}
% \begin{tabularx}{\linewidth}{cYYYYYYYYYYYY}
% \toprule %\hline
% \multirow{2}{*}{Model} & \multicolumn{6}{c}{Gowalla} & \multicolumn{6}{c}{SIN}\\ 
% \cmidrule[0.5pt](lr){2-7}\cmidrule[0.5pt](lr){8-13}
% & R@2 & R@5 & R@10 & N@2 & N@5 & N@10 & R@2 & R@5 & R@10 & N@2 & N@5 & N@10\\
% \midrule
% MF & 0.0414 & 0.0869 & 0.1473 & & & 0.1087 & 0.1103 & 0.1766 & 0.2059 & & &  0.0868\\ %& 0.2896 & 0.3141 & 0.3866 & 0.2327 & 0.2361 & 0.2792 & 0.3046 & 0.2426\\
% LightGCN & 0.1082 & 0.1348 & 0.1699 & & & 0.1432 & 0.1606 & 0.2144 & 0.2419 & & & 0.1892\\ % & 0.3917 & 0.4473 & 0.4936 & 0.4403 & 0.3789 & 0.4363 & 0.4519 & 0.3903\\
% DGCF & 0.1147 & 0.1396 & 0.1721 & & & 0.1561 & 0.1798 & 0.2040 & 0.2285 & & & 0.2269\\ %& 0.4204 & 0.4913 & 0.5310 & 0.4558 & 0.3368 & 0.4167 & 0.5653 & 0.5041\\
% \midrule
% GeoIE & 0.1767 & 0.2123 & 0.2436 & & & 0.1929 & 0.2521 & 0.2867 & 0.3162 & &  & 0.2679 \\ % & 0.4975 & 0.5408 & 0.5726 & 0.5141 & 0.5655 & 0.5994 & 0.6251 & 0.5805 \\
% LSTPM & 0.1948 & 0.2049 & 0.2618 & & & 0.1742 & 0.2704 & 0.3253 & 0.3791 & & & 0.2749 \\ %& 0.5029 & 0.5513 & 0.5795 & 0.4962 & 0.5754 & 0.6020 & 0.6312 & 0.5681\\
% STAN & \underline{0.2195} & 0.2364 & 0.2994 & & & 0.2268 & 0.2634 & 0.2940 & 0.3208 & & &  0.2892\\  %& & & & & \underline{0.6027} & \underline{0.6358} & \underline{0.6533} & \underline{0.6124} \\
% \midrule
% SGRec & \\
% DRAN & 0.2133 & \underline{0.2466} & \underline{0.3056} & &  & \underline{0.2367} & \underline{0.3086} & \underline{0.3554} & \underline{0.3921} & & &  \underline{0.3297} \\ % & \underline{0.5225} & \underline{0.5770} & \underline{0.6210} & \underline{0.5602} & {0.5859} & {0.6253} & {0.6478} & {0.5956}\\
% \midrule
% \method{} & \textbf{0.2685\textsuperscript{$\star$}} & \textbf{0.3086\textsuperscript{$\star$}} & \textbf{0.3421\textsuperscript{$\star$}} & & &  \textbf{0.2872\textsuperscript{$\star$}} & \textbf{0.3455\textsuperscript{$\star$}} & \textbf{0.3906\textsuperscript{$\star$}} & \textbf{0.4294\textsuperscript{$\star$}} & & &  \textbf{0.3649\textsuperscript{$\star$}}\\ % & \textbf{0.5951\textsuperscript{$\star$}} & \textbf{0.6341\textsuperscript{$\star$}} & \textbf{0.6611\textsuperscript{$\star$}} & \textbf{0.6090\textsuperscript{$\star$}} & \textbf{0.6146\textsuperscript{$\star$}} & \textbf{0.6422\textsuperscript{$\star$}} & \textbf{0.6632\textsuperscript{$\star$}} & \textbf{0.6253\textsuperscript{$\star$}} \\
% Improv. & \\
% \bottomrule % \hline
% \end{tabularx}
% \end{table*}



% \begin{table*}
% \centering
% \caption{The test results on TKY and NYC.}
% \label{tab:overall_2}
% \begin{tabularx}{\linewidth}{cYYYYYYYYYYYY}
% \toprule %\hline
% \multirow{2}{*}{Model} & \multicolumn{6}{c}{TKY} & \multicolumn{6}{c}{NYC}\\ 
% \cmidrule[0.5pt](lr){2-7}\cmidrule[0.5pt](lr){8-13}
% & R@2 & R@5 & R@10 & N@2 & N@5 & N@10 & R@2 & R@5 & R@10 & N@2 & N@5 & N@10\\
% \midrule
% MF & 0.2896 & 0.3141 & 0.3866 & & & 0.2327 & 0.2361 & 0.2792 & 0.3046 &  & & 0.2426\\
% LightGCN & 0.3917 & 0.4473 & 0.4936 & &  & 0.4403 & 0.3789 & 0.4363 & 0.4519 &  & & 0.3903\\
% DGCF & 0.4204 & 0.4913 & 0.5310 & & &  0.4558 & 0.3368 & 0.4167 & 0.5653 & & &  0.5041\\
% \midrule
% GeoIE & 0.4975 & 0.5408 & 0.5726  & & & 0.5141 & 0.5655 & 0.5994 & 0.6251 &  & & 0.5805 \\
% LSTPM & 0.5029 & 0.5513 & 0.5795 & & &  0.4962 & 0.5754 & 0.6020 & 0.6312 &  & & 0.5681\\
% STAN & & & & & &  & \underline{0.6027} & \underline{0.6358} & \underline{0.6533} &  & & \underline{0.6124} \\
% \midrule
% SGRec & \\
% DRAN & \underline{0.5225} & \underline{0.5770} & \underline{0.6210} & & &  \underline{0.5602} & {0.5859} & {0.6253} & {0.6478} & & &  {0.5956}\\
% \midrule
% \method{} & \textbf{0.5951\textsuperscript{$\star$}} & \textbf{0.6341\textsuperscript{$\star$}} & \textbf{0.6611\textsuperscript{$\star$}} &  & & \textbf{0.6090\textsuperscript{$\star$}} & \textbf{0.6146\textsuperscript{$\star$}} & \textbf{0.6422\textsuperscript{$\star$}} & \textbf{0.6632\textsuperscript{$\star$}} &  & & \textbf{0.6253\textsuperscript{$\star$}} \\
% Improv. & \\
% \bottomrule % \hline
% \end{tabularx}
% \end{table*}

% \begin{table*}
% \centering
% \caption{The test results of \method{} and all baselines, where R@K and N@K are short for Recall@K and NDCG@K. The highest performance is emphasized with bold font and the second highest is marked with underlines.\textbf{$\star$} indicates that \method{} outperforms the best baseline model at a p-value<0.05 level of unpaired t-test.}
% \label{tab:overall}
% \begin{tabularx}{\linewidth}{cYYYYYYYYYYYYYYYY}
% \toprule %\hline
% \multirow{2}{*}{Model} & \multicolumn{4}{c}{Gowalla} & \multicolumn{4}{c}{SIN}  & \multicolumn{4}{c}{TKY}  & \multicolumn{4}{c}{NYC} \\ 
% \cmidrule[0.5pt](lr){2-5}\cmidrule[0.5pt](lr){6-9}\cmidrule[0.5pt](lr){10-13}\cmidrule[0.5pt](lr){14-17}
% & R@2 & R@5 & R@10 & N@10 & R@2 & R@5 & R@10 & N@10 & R@2 & R@5 & R@10 & N@10 & R@2 & R@5 & R@10 & N@10\\
% \midrule
% MF & 0.0414 & 0.0869 & 0.1473 & 0.1087 & 0.1103 & 0.1766 & 0.2059 & 0.0868 & 0.2896 & 0.3141 & 0.3866 & 0.2327 & 0.2361 & 0.2792 & 0.3046 & 0.2426\\
% LightGCN & 0.1082 & 0.1348 & 0.1699 & 0.1432 & 0.1606 & 0.2144 & 0.2419 & 0.1892 & 0.3917 & 0.4473 & 0.4936 & 0.4403 & 0.3789 & 0.4363 & 0.4519 & 0.3903\\
% DGCF & 0.1147 & 0.1396 & 0.1721 & 0.1561 & 0.1798 & 0.2040 & 0.2285 & 0.2269 & 0.4204 & 0.4913 & 0.5310 & 0.4558 & 0.3368 & 0.4167 & 0.5653 & 0.5041\\
% \midrule
% GeoIE & 0.1767 & 0.2123 & 0.2436 & 0.1929 & 0.2521 & 0.2867 & 0.3162 & 0.2679 & 0.4975 & 0.5408 & 0.5726 & 0.5141 & 0.5655 & 0.5994 & 0.6251 & 0.5805 \\
% LSTPM & 0.1948 & 0.2049 & 0.2618 & 0.1742 & 0.2704 & 0.3253 & 0.3791 & 0.2749 & 0.5029 & 0.5513 & 0.5795 & 0.4962 & 0.5754 & 0.6020 & 0.6312 & 0.5681\\
% STAN & \underline{0.2195} & 0.2364 & 0.2994 & 0.2268 & 0.2634 & 0.2940 & 0.3208 & 0.2892 & & & & & \underline{0.6027} & \underline{0.6358} & \underline{0.6533} & \underline{0.6124} \\
% \midrule
% SGRec & \\
% DRAN & 0.2133 & \underline{0.2466} & \underline{0.3056} & \underline{0.2367} & \underline{0.3086} & \underline{0.3554} & \underline{0.3921} & \underline{0.3297} & \underline{0.5225} & \underline{0.5770} & \underline{0.6210} & \underline{0.5602} & {0.5859} & {0.6253} & {0.6478} & {0.5956}\\
% \midrule
% \method{} & \textbf{0.2685\textsuperscript{$\star$}} & \textbf{0.3086\textsuperscript{$\star$}} & \textbf{0.3421\textsuperscript{$\star$}} & \textbf{0.2872\textsuperscript{$\star$}} & \textbf{0.3455\textsuperscript{$\star$}} & \textbf{0.3906\textsuperscript{$\star$}} & \textbf{0.4294\textsuperscript{$\star$}} & \textbf{0.3649\textsuperscript{$\star$}} & \textbf{0.5951\textsuperscript{$\star$}} & \textbf{0.6341\textsuperscript{$\star$}} & \textbf{0.6611\textsuperscript{$\star$}} & \textbf{0.6090\textsuperscript{$\star$}} & \textbf{0.6146\textsuperscript{$\star$}} & \textbf{0.6422\textsuperscript{$\star$}} & \textbf{0.6632\textsuperscript{$\star$}} & \textbf{0.6253\textsuperscript{$\star$}} \\
% Improv. & \\
% \bottomrule % \hline
% \end{tabularx}
% \end{table*}

